Balanced Multi-modal Federated Learning via Cross-Modal Infiltration

Federated learning (FL) underpins advancements in privacy-preserving distributed computing by collaboratively training neural networks without exposing clients' raw data. Current FL paradigms primarily focus on uni-modal data, while exploiting the knowledge from distributed multimodal data remains largely unexplored. Existing multimodal FL (MFL) solutions are mainly designed for statistical or modality heterogeneity from the input side, however, have yet to solve the fundamental issue,"modality imbalance", in distributed conditions, which can lead to inadequate information exploitation and heterogeneous knowledge aggregation on different modalities.In this paper, we propose a novel Cross-Modal Infiltration Federated Learning (FedCMI) framework that effectively alleviates modality imbalance and knowledge heterogeneity via knowledge transfer from the global dominant modality. To avoid the loss of information in the weak modality due to merely imitating the behavior of dominant modality, we design the two-projector module to integrate the knowledge from dominant modality while still promoting the local feature exploitation of weak modality. In addition, we introduce a class-wise temperature adaptation scheme to achieve fair performance across different classes. Extensive experiments over popular datasets are conducted and give us a gratifying confirmation of the proposed framework for fully exploring the information of each modality in MFL.

==> sec/3_analysis.tex <==
\section{Observations and Analysis}
\label{sec:analysis}

Intuitively, we should use as more data as possible for each client to capture the comprehensive information, especially for multi-modal FL due to the complementary features between different modalities. However, we make the counter-intuitive observation as shown in \cref{fig:drop comparison}. We perform the pre-experiment on CREMA-D \cite{cao2014crema} (an audio-visual dataset for emotion recognition) with uniformly distributed data on 20 clients. Then, we randomly discard the data of one modality (audio or visual) on the clients with a certain probability and find that discarding some modalities for part of clients does not necessarily lead to performance degradation of the global model, but may lead to an improvement in performance.

To explore the cause behind, we demonstrate the performance of each modality as shown in \cref{fig:uni-audio performance comparison,fig:uni-visual performance comparison}. It is clear that audio performs much better than visual when there is no data deprecation (FedAvg), but the gap between them gradually narrows as the modal drop probability increases until visual performs better than audio (FedAvg-0.2). This phenomenon can be explained by `modality imbalance': audio dominants the multi-modal learning while the visual modality is extremely inhibited;  when we abandon the audio data in some clients, the potential of visual modality is released and the global model gets improvement by absorbing the released information through aggregation.

Motivated by these observations, we intend to design a modality selection method, a new scheme in MFL that selects appropriate data in each client to participate in each round of training to address underutilization of information and global performance degradation. As we can see in \cref{fig:motivation experiment}, discarding audio data can do achieve some improvement for visual modality while it also reduces the accuracy of audio modality, which may still lead to performance degradation of global model. Therefore, we should consider keeping a balance between information exploration and contribution to the aggregated model. 







